Parton distribution functions of $\Delta^+$ on the lattice

We perform a first calculation for the unpolarized parton distribution function of the $\Delta^+$ baryon using lattice QCD simulations within the framework of Large Momentum Effective Theory. Two ensembles of $N_f=2+1+1$ twisted mass fermions are utilized with a pion mass of 270 MeV and 360 MeV, respectively. The baryon, which is treated as a stable single-particle state, is boosted with momentum $P_3$ with values $\{0.42,0.83,1.25\}$ GeV, and we utilize momentum smearing to improve the signal. The unpolarized parton distribution function of $\Delta^+$ is obtained using a non-perturbative renormalization and a one-loop formula for the matching, with encouraging precision. In particular, we compute the $\overline{d}(x)-\overline{u}(x)$ asymmetry and compare it with the same quantity in the nucleon, in a first attempt towards resolving the physical mechanism responsible for generating such asymmetry.

==> Proofs.tex <==
Dear production team below you will find comments on the proofs we received for article DQ12392.


Comment 1:
----------

line 305: please replace "procedure relies on an RI$'$ scheme" with procedure relies on a regularization independent scheme (RI$'$)"

line 353: please replace "The conversion to the $\overline{\rm MS}$" with "The conversion to the minimal subtraction scheme ($\overline{\rm MS}$)"

Comment 2:
----------
The funding information is correct.

Comment 3:
----------
The references 65 and 68 are correct

Comment 4:
----------
We prefer that all authors are shown in Ref. 4, 41, 67, 72,  and 80. The bibitems are:

Ref. 4:
\bibitem[{\citenamefont{Alexandrou
  et~al.}(2019{\natexlab{c}})\citenamefont{Alexandrou, Bacchio, Constantinou,
  Dimopoulos, Finkenrath, Frezzotti, Hadjiyiannakou, Jansen, Kostrzewa, Koutsou
  et~al.}}]{Alexandrou:2019ali}
\bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Alexandrou}},
  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Bacchio}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Constantinou}},
  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Dimopoulos}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Finkenrath}},
  \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Frezzotti}},
  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Hadjiyiannakou}},
  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Jansen}},
  \bibinfo{author}{\bibfnamefont{B.}~\bibnamefont{Kostrzewa}},
  \bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Koutsou}},
  \bibnamefont{et~al.} (\bibinfo{year}{2019}{\natexlab{c}}),
  \eprint{1908.10706}.
  
Ref. 41:  
  \bibitem[{\citenamefont{Liu et~al.}(2018{\natexlab{a}})\citenamefont{Liu, Chen,
  Huo, Jin, Schlemmer, Schaefer, Sun, Wang, Yang, Zhang et~al.}}]{Liu:2018uuj}
\bibinfo{author}{\bibfnamefont{Y.-S.} \bibnamefont{Liu}},
  \bibinfo{author}{\bibfnamefont{J.-W.} \bibnamefont{Chen}},
  \bibinfo{author}{\bibfnamefont{Y.-K.} \bibnamefont{Huo}},
  \bibinfo{author}{\bibfnamefont{L.}~\bibnamefont{Jin}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Schlemmer}},
  \bibinfo{author}{\bibfnamefont{A.}~\bibnamefont{Schaefer}},
  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Sun}},
  \bibinfo{author}{\bibfnamefont{W.}~\bibnamefont{Wang}},
  \bibinfo{author}{\bibfnamefont{Y.-B.} \bibnamefont{Yang}},
  \bibinfo{author}{\bibfnamefont{J.-H.} \bibnamefont{Zhang}},
  \bibnamefont{et~al.} (\bibinfo{year}{2018}{\natexlab{a}}),
  \eprint{1807.06566}.
  
Ref. 67:
  \bibitem[{\citenamefont{Alexandrou
  et~al.}(2018{\natexlab{c}})\citenamefont{Alexandrou, Bacchio, Charalambous,
  Dimopoulos, Finkenrath, Frezzotti, Hadjiyiannakou, Jansen, Koutsou, Kostrzewa
  et~al.}}]{Alexandrou:2018egz}
\bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Alexandrou}},
  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Bacchio}},
  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Charalambous}},
  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Dimopoulos}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Finkenrath}},
  \bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Frezzotti}},
  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Hadjiyiannakou}},
  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Jansen}},
  \bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Koutsou}},
  \bibinfo{author}{\bibfnamefont{B.}~\bibnamefont{Kostrzewa}},
  \bibnamefont{et~al.}, \bibinfo{journal}{Phys. Rev.}
  \textbf{\bibinfo{volume}{D98}}, \bibinfo{pages}{054518}
  (\bibinfo{year}{2018}{\natexlab{c}}), \eprint{1807.00495}.
  
Ref. 72:  
  \bibitem[{\citenamefont{Alexandrou et~al.}(2008)\citenamefont{Alexandrou,
  Baron, Blossier, Brinet, Carbonell, Dimopoulos, Drach, Farchioni, Frezzotti,
  Guichon et~al.}}]{Alexandrou:2008tn}
\bibinfo{author}{\bibfnamefont{C.}~\bibnamefont{Alexandrou}},
  \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Baron}},
  \bibinfo{author}{\bibfnamefont{B.}~\bibnamefont{Blossier}},
  \bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Brinet}},
  \bibinfo{author}{\bibfnamefont{J.}~\bibnamefont{Carbonell}},
  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Dimopoulos}},
  \bibinfo{author}{\bibfnamefont{V.}~\bibnamefont{Drach}},
  \bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Farchioni}},
  \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Frezzotti}},
  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Guichon}},
  \bibnamefont{et~al.} (\bibinfo{collaboration}{European Twisted Mass}),
  \bibinfo{journal}{Phys. Rev.} \textbf{\bibinfo{volume}{D78}},
  \bibinfo{pages}{014509} (\bibinfo{year}{2008}), \eprint{0803.3190}.
  

Ref. 80:
  \bibitem[{\citenamefont{Constantinou et~al.}(2010)\citenamefont{Constantinou,
  Dimopoulos, Frezzotti, Herdoiza, Jansen, Lubicz, Panagopoulos, Rossi, Simula,
  Stylianou et~al.}}]{Constantinou:2010gr}
\bibinfo{author}{\bibfnamefont{M.}~\bibnamefont{Constantinou}},
  \bibinfo{author}{\bibfnamefont{P.}~\bibnamefont{Dimopoulos}},
  \bibinfo{author}{\bibfnamefont{R.}~\bibnamefont{Frezzotti}},
  \bibinfo{author}{\bibfnamefont{G.}~\bibnamefont{Herdoiza}},
  \bibinfo{author}{\bibfnamefont{K.}~\bibnamefont{Jansen}},
  \bibinfo{author}{\bibfnamefont{V.}~\bibnamefont{Lubicz}},
  \bibinfo{author}{\bibfnamefont{H.}~\bibnamefont{Panagopoulos}},
  \bibinfo{author}{\bibfnamefont{G.~C.} \bibnamefont{Rossi}},
  \bibinfo{author}{\bibfnamefont{S.}~\bibnamefont{Simula}},
  \bibinfo{author}{\bibfnamefont{F.}~\bibnamefont{Stylianou}},
  \bibnamefont{et~al.} (\bibinfo{collaboration}{ETM}), \bibinfo{journal}{JHEP}
  \textbf{\bibinfo{volume}{08}}, \bibinfo{pages}{068} (\bibinfo{year}{2010}),
  \eprint{1004.1115}.
